On the Shuffle Automaton Size for Words

We investigate the state size of DFAs accepting the shuffle of two words. We provide words u and v, such that the minimal DFA for u shuffled with v requires an exponential number of states. We also show some conditions for the words u and v which ensure a quadratic upper bound on the state size of u shuffled with v. Moreover, switching only two letters within one of u or v is enough to trigger the change from quadratic to exponential.

==> dcfs.tex <==
\usepackage{amssymb,amsmath}
\makeatletter
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{problem}[theorem]{Problem}
\newtheorem{definition}[theorem]{Definition\dromanb}
\newtheorem{remark}[theorem]{Remark\dromanb}
\newtheorem{example}[theorem]{Example\dromanb}
\newtheorem{claim}{\itshape Claim\d@cproof}
\newcommand*{\dromanb}{\gdef\d@tstyle{\rmfamily\upshape\mdseries}}

\newcommand{\d@tstyle}{}
\renewcommand{\@begintheorem}[2]{%
  \par\gdef\d@tstyle{\rmfamily\itshape\mdseries}\trivlist
  \item[\hskip\labelsep{\rmfamily\upshape\bfseries
    #1\ #2.}]\d@tstyle\ignorespaces}
\renewcommand{\@opargbegintheorem}[3]{%
  \par\gdef\d@tstyle{\rmfamily\itshape\mdseries}\trivlist
  \item[\hskip\labelsep{\rmfamily\upshape\bfseries
    #1\ #2\hskip\labelsep #3.}]\d@tstyle\ignorespaces}
\newcounter{d@proof}\let\thed@proof\relax\setcounter{d@proof}{0}
\newcommand*{\d@cproof}{%
  \ifnum \value{d@proof}=0{\@warning{\protect\begin{claim} ...
    \protect\end{claim} not nested in any `proof'^^J or `proofof'
    environment,}}\else\fi
}

%\newcommand*{\qed}{\raisebox{0.5ex}[0ex][0ex]{\framebox[1ex][l]{}}}
\newcommand*{\qed}{$\Box$}

\newenvironment{proof}{%
  \ifnum \value{d@proof}=0{\setcounter{claim}{0}}\else\fi
  \stepcounter{d@proof}\par\noindent
  {\rmfamily\itshape\mdseries Proof\/}:\hspace{\labelsep}\ignorespaces}%
  {\addtocounter{d@proof}{-1}\mbox{}\nolinebreak\hfill~%
  \ifnum \value{d@proof}=0{\qed}\else
    \ifnum \value{d@proof}=1{\qed\nolinebreak\,\nolinebreak\qed}\else
      \ifnum \value{d@proof}=2{\qed\nolinebreak\,\nolinebreak\qed
          \nolinebreak\,\nolinebreak\qed}\else
        {\qed\nolinebreak...\nolinebreak\qed}%
  \fi\fi\fi
  \medbreak
}
\newenvironment{proofof}[1]{%
  \vspace{\parskip}\vspace{\topsep}\vspace{\partopsep}%
  \ifnum \value{d@proof}=0{\setcounter{claim}{0}}\else\fi
  \stepcounter{d@proof}\par\noindent
  {\rmfamily\upshape\bfseries Proof of #1.}\hspace{\labelsep}\ignorespaces}%
  {\addtocounter{d@proof}{-1}\mbox{}\nolinebreak\hfill~%
  \ifnum \value{d@proof}=0{\qed}\else
    \ifnum \value{d@proof}=1{\qed\nolinebreak\,\nolinebreak\qed}\else
      \ifnum \value{d@proof}=2{\qed\nolinebreak\,\nolinebreak\qed
          \nolinebreak\,\nolinebreak\qed}\else
        {\qed\nolinebreak...\nolinebreak\qed}%
  \fi\fi\fi
  \medbreak
}
\newenvironment{proof*}{%
  \ifnum \value{d@proof}=0{\setcounter{claim}{0}}\else\fi
  \par\noindent
  {\rmfamily\itshape\mdseries Proof\/}:\hspace{\labelsep}\ignorespaces}%
  {
}
\makeatother

\setlength{\arraycolsep}{2.3pt}


==> eptcsdata.tex <==
\providecommand{\event}{J.~Dassow, G.~Pighizzini, B.~Truthe (Eds.): 11th International Workshop\\
on Descriptional Complexity of Formal Systems (DCFS 2009)}
\providecommand{\volume}{3}
\providecommand{\anno}{2009}
\providecommand{\firstpage}{79}
\providecommand{\eid}{7}

